No Strong Feelings One Way or Another: Re-operationalizing Neutrality in Natural Language Inference

Natural Language Inference (NLI) has been a cornerstone task in evaluating language models' inferential reasoning capabilities. However, the standard three-way classification scheme used in NLI has well-known shortcomings in evaluating models' ability to capture the nuances of natural human reasoning. In this paper, we argue that the operationalization of the neutral label in current NLI datasets has low validity, is interpreted inconsistently, and that at least one important sense of neutrality is often ignored. We uncover the detrimental impact of these shortcomings, which in some cases leads to annotation datasets that actually decrease performance on downstream tasks. We compare approaches of handling annotator disagreement and identify flaws in a recent NLI dataset that designs an annotator study based on a problematic operationalization. Our findings highlight the need for a more refined evaluation framework for NLI, and we hope to spark further discussion and action in the NLP community.

==> latex/discussion.tex <==
\section{Discussion}\label{sec:discussion}
Although we have highlighted issues with UNLI in this paper, similar problems in operationalization and psychometric practices are not unique to UNLI, nor even to NLI. We conclude our analysis by broadly reviewing select issues in popular NLI datasets.

\paragraph{Bias in Instructions}
The majority of NLI datasets have relied on human annotators for their development. While this has enabled the creation of large-scale NLI datasets \cite{Bowman_Angeli_Potts_Manning_2015}, it also introduces the possibility of artifacts in the data that may lead to models easily achieving high performance. \citet{Gururangan_Swayamdipta_Levy_Schwartz_Bowman_Smith_2018} investigated such biases and found that high accuracy could be achieved on both SNLI and MultiNLI using a hypothesis-only classifier. This was attributed to biases introduced by the annotators, such as overuse of gender-neutral references, presumably to speed up the task. \citet{elazar2020extraordinary} observed low inter-annotator agreement when using the protocol designed by \citet{Bowman_Angeli_Potts_Manning_2015} to build an NLI dataset for testing complement coercion. The low agreement was attributed to ambiguous situations in items, which was exacerbated by typical instructions in NLI datasets that leave the correct annotation up to the worker's ``commonsense.'' Other studies have also found that the focus on creating simple annotation guidelines can be detrimental, leading to confusion among workers about how to label items \cite{kalouli2019explaining,parmar2022don}. In summary, previous research has revealed that efforts to facilitate large-scale annotation studies in NLI have led to unintended consequences such as unclear task instructions, resulting in low agreement among annotators and the propagation of undesired biases. \citet{mcdonnell2016relevant,Borin_2022} argue that asking annotators for explanations can help enforce data quality.

\paragraph{Number of Annotators}
The two most widely used NLI datasets, SNLI \cite{Bowman_Angeli_Potts_Manning_2015} and MultiNLI \cite{Williams_Nangia_Bowman_2018}, provide annotations from five annotators for their dev and test sets and one annotation for their train sets.\footnote{SNLI has very few items in its train set with more than one annotation.} \citet{nie-etal-2020-learn} later took subsets of SNLI and MultiNLI dev sets and elicited 100 annotations for each item. They found that the majority label with 100 annotations was different than the majority label reported in SNLI and MultiNLI for $20\%$ and $31\%$ of the items respectively. Newer NLI datasets like ANLI \cite{Nie_Williams_Dinan_Bansal_Weston_Kiela_2020} and UNLI \cite{chen-etal-2020-uncertain} report even fewer than five annotations, with UNLI failing to report the two annotations they gathered for each item (Section \ref{sec:unli}). With so few annotations, measuring reliability and using the datasets for other downstream tasks becomes difficult. An instance of this problem occurs in this very paper, where we wanted to train a model for predicting inter-annotator agreement on NLI datasets but were limited only to a few examples from SNLI, MultiNLI, and ChaosNLI.


